Models for Metal Hydride Particle Shape, Packing, and Heat Transfer

A multiphysics modeling approach for heat conduction in metal hydride powders is presented, including particle shape distribution, size distribution, granular packing structure, and effective thermal conductivity. A statistical geometric model is presented that replicates features of particle size and shape distributions observed experimentally that result from cyclic hydride decreptitation. The quasi-static dense packing of a sample set of these particles is simulated via energy-based structural optimization methods. These particles jam (i.e., solidify) at a density (solid volume fraction) of 0.665+/-0.015 - higher than prior experimental estimates. Effective thermal conductivity of the jammed system is simulated and found to follow the behavior predicted by granular effective medium theory. Finally, a theory is presented that links the properties of bi-porous cohesive powders to the present systems based on recent experimental observations of jammed packings of fine powder. This theory produces quantitative experimental agreement with metal hydride powders of various compositions.

==> complatexnom <==
latex vc_nomenclature
makeindex vc_nomenclature.nlo -s nomencl.ist -o vc_nomenclature.nls
bibtex vc_nomenclature
sed -i 's/(????)//g' vc_nomenclature.bbl
sed -i 's/, ????/./g' vc_nomenclature.bbl
sed -i 's/newblock ????/newblock/g' vc_nomenclature.bbl
sed -i 's/\/xfnm\[\]//g' vc_nomenclature.bbl
latex vc_nomenclature
latex vc_nomenclature
dvipdf vc_nomenclature

